Software frameworks for integral equations in electromagnetic scattering based on Calder\'on identities

In recent years there have been tremendous advances in the theoretical understanding of boundary integral equations for Maxwell problems. In particular, stable dual pairing of discretisation spaces have been developed that allow robust formulations of the preconditioned electric field, magnetic field and combined field integral equations. Within the BEM++ boundary element library we have developed implementations of these frameworks that allow an intuitive formulation of the typical Maxwell boundary integral formulations within a few lines of code. The basis of these developments is an efficient and robust implementations of Calder\'on identities together with a product algebra that hides and automates most technicalities involved in assembling Galerkin boundary integral equations. In this paper we demonstrate this framework and use it to derive very simple and robust software formulations of the standard preconditioned electric field, magnetic field and regularised combined field integral equations for Maxwell.

==> img/cfie_iterations.tex <==
% This file was created by matplotlib2tikz v0.5.15.
\begin{tikzpicture}

\begin{axis}[
xlabel={Number of edges in grid},
ylabel={Number of GMRES iterations},
xmin=54, xmax=18765,
ymin=8, ymax=10000,
ymode=log,
xmode=log,
axis on top
]
\cfieplot
table {%
72 11
348 11
954 11
3198 10
12510 9
};
\end{axis}

\end{tikzpicture}


==> img/efie_calderon_iteration_count.tex <==
% This file was created by matplotlib2tikz v0.5.15.
\begin{tikzpicture}

\begin{axis}[
xlabel={Number of edges in grid},
ylabel={Number of GMRES iterations},
xmin=54, xmax=18765,
ymin=8, ymax=10000,
ymode=log,
xmode=log,
axis on top
]
\efieplot
table {%
72 34
348 105
954 203
3198 532
12510 1395
};
\calefieplot
table {%
72 10
348 11
954 11
3198 11
12510 10
};
\end{axis}

\end{tikzpicture}


==> img/mfie_iteration_count.tex <==
% This file was created by matplotlib2tikz v0.5.15.
\begin{tikzpicture}

\begin{axis}[
xlabel={Number of unknowns},
ylabel={Number of GMRES iterations},
xmin=54, xmax=18765,
ymin=8, ymax=10000,
ymode=log,
xmode=log,
axis on top
]
\mfieplot
table {%
72 12
348 13
954 13
3198 12
12510 10
};
\badmfieplot
table {%
72 720
348 3480
1000 10001
};
\end{axis}

\end{tikzpicture}

